Uncertainty-aware Human Mobility Modeling and Anomaly Detection

Given the temporal GPS coordinates from a large set of human agents, how can we model their mobility behavior toward effective anomaly (e.g. bad-actor or malicious behavior) detection without any labeled data? Human mobility and trajectory modeling have been extensively studied, showcasing varying abilities to manage complex inputs and balance performance-efficiency trade-offs. In this work, we formulate anomaly detection in complex human behavior by modeling raw GPS data as a sequence of stay-point events, each characterized by spatio-temporal features, along with trips (i.e. commute) between the stay-points. Our problem formulation allows us to leverage modern sequence models for unsupervised training and anomaly detection. Notably, we equip our proposed model USTAD (for Uncertainty-aware Spatio-Temporal Anomaly Detection) with aleatoric (i.e. data) uncertainty estimation to account for inherent stochasticity in certain individuals' behavior, as well as epistemic (i.e. model) uncertainty to handle data sparsity under a large variety of human behaviors. Together, aleatoric and epistemic uncertainties unlock a robust loss function as well as uncertainty-aware decision-making in anomaly scoring. Extensive experiments shows that USTAD improves anomaly detection AUCROC by 3\%-15\% over baselines in industry-scale data.

==> 05deployment.tex <==


% In this section, we discuss how the can be deployed in real network planning and optimization scenarios. 
% The platform integrates multiple teams and components, including mobility simulation teams responsible for generating realistic mobility data and downstream task teams that focus on pattern learning, prediction, and anomaly detection.
\method has been deployed on the Novateur AI Platform, a system designed for human mobility analysis, modeling, simulation and anomaly detection. The framework of the platform is illustrated in Figure~\ref{fig:sys_framework}, where \method plays a critical role in human mobility anomaly detection (highlighted in red).
To evaluate the performance of the deployed \method,  we conducted anomaly detection on the same 20K agents in the \trial dataset, generated by Novateur's simulation system. We compared \method against Novateur's existing online model (called \ssmlp, see Appx \ref{appendix:anomaly_detection_baselines} for details). 

\textbf{Performance Gains:} \method significantly outperforms \ssmlp, achieving a 20\% increase in AUCROC and a 118\% increase in AUPR for agent-level anomaly detection, as well as a 41\% increase in AUCROC and a 259\% increase in AUPR for event-level anomaly detection.
Beyond performance gains, \method introduces a self-improving feedback loop within the system. By identifying unrealistic anomalies (e.g., having lunch for 2 days), \method helps refine the simulation system, enabling it to generate more challenging and realistic anomalies in subsequent iterations.
This continuous refinement enhances both the quality of the simulations and the accuracy of anomaly detection.
% teleportation events
%This continuous refinement enhances both the quality of the simulations and the robust evaluation of anomaly detection.

% (e.g., having lunch for 2 days)


%By reporting overly unrealistic anomalies (e.g. teleportation), the simulation system would refine the anomaly injection process to generate more challenging and realistic anomalies in subsequent iterations. 


%The performance improvement of anomaly detection would encourage the simulation system to generate more complex and challenging behavior data. Such ``adversarial'' refinement process can finally lead to improvement in simulations and robustness of anomaly detection.

%By reporting overly unrealistic anomalies (e.g. ), the simulation system would refine the anomaly injection process to generate more challenging and realistic anomalies in subsequent iterations. This continuous refinement enhances both the realism of the simulations and the robustness of anomaly detection.
%, highlighting \method's value within the system and its potential to advance human mobility understanding.

% The performance improvement of anomaly detection would encourage the simulation system to generate more complex and challenging behavior data. Such ``adversarial'' refinement process can finally lead to improvement in simulations and robustness of anomaly detection.

%Motivated by the promising results, we deploy \method on Novateur to test its performance online. Specifically, we select the same 20k agents in \trialthree generated by Novateur's simulation system, then conduct the anomaly detection to compare \method and Novateur's current online model (called \ssmlp, details can be found in Appx \ref{appendix:anomaly_detection_baselines}). From the results of the A/B test, \method gains 7.4\% improvement in AUCROC and 118.1\% in AUPR in anomaly detection.


\begin{figure}[htbp]
 \vspace{-0.05in}
  \includegraphics[width= 1\linewidth]{img/Deployment Pipeline.pdf}
   \vspace{-2.2em}
  \caption{Framework of Novateur AI Platform.}
  \label{fig:sys_framework}
  \vspace{-2.5em}
\end{figure}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/tab_AD_full.tex <==
\begin{table*}[!th]
    \caption{Anomaly detection results at the event-level (left) and the  agent-level (right).}
    \vspace{-0.1in}
    \centering
    \renewcommand\arraystretch{1.1}
    \setlength\tabcolsep{2 pt}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{c|cc|cc|cc||cc|cc|cc}
    \toprule
        \multirow{2}{*}{Method} & \multicolumn{6}{c||}{Event-level Anomaly Detection} & \multicolumn{6}{c}{Agent-level Anomaly Detection}  \\
        \cline{2-13}
         & \multicolumn{2}{|c|}{\trial(small)} & \multicolumn{2}{|c|}{\NUMOSIM(small)} & \multicolumn{2}{|c||}{\NUMOSIM(20K)} & \multicolumn{2}{|c|}{\trial(small)} & \multicolumn{2}{|c|}{\NUMOSIM(small)} & \multicolumn{2}{|c}{\NUMOSIM(20K)}  \\
        \cline{2-13}
         & AUROC & AUPR & AUROC & AUPR & AUROC & AUPR & AUROC & AUPR & AUROC & AUPR & AUROC & AUPR \\
         \midrule
         STOD & 0.577 & 0.073 & 0.571 & 0.071 & 0.584 & 0.003 & 0.506 & 0.655 & 0.511 & 0.468 & 0.519 & 0.020 \\
          RioBus & 0.503 & 0.044 & 0.530 & 0.047 & 0.532 & 0.002 & 0.488 & 0.632 & 0.510 & 0.453 & 0.508 & 0.019 \\
          SS-MLP & 0.596 & 0.172 & 0.630& \underline{0.144} & 0.634& 0.008 & 0.653 & 0.777 & \textbf{0.697} & \textbf{0.638} & 0.703 & 0.053 \\
         LSTM & \underline{0.755} & 0.182 & \underline{0.637} & 0.122 & \underline{0.642} & 0.020 & 0.631 & 0.706 & 0.599 & 0.526 & 0.658 & 0.062 \\
         Transformer & 0.723 & \underline{0.232} & 0.635 & 0.132 & 0.636 & \underline{0.033} & \underline{0.679} & \underline{0.785} & 0.625 & 0.525 & \underline{0.717} & \underline{0.095} \\
         \midrule
         \method & \textbf{0.795} & \textbf{0.329} & \textbf{0.694} & \textbf{0.146} & \textbf{0.670} & \textbf{0.034} & \textbf{0.746} & \textbf{0.841} & \underline{0.655} & \underline{0.572} & \textbf{0.727} & \textbf{0.114} \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.1in}
    \label{tab:anomaly_detection}
\end{table*}



==> tables/tab_AD_score_func.tex <==

% \begin{table}% 'r' for right, 'l' for left, width of the figure
%     \caption{Comparison of different anomaly scoring functions for event-level detection. \blue{Agent-level comparison can be found in Table}}
%     \vspace{-0.1in}
%     \centering
%     \renewcommand\arraystretch{1.1}
%     \setlength\tabcolsep{2 pt}
%     \resizebox{0.6\linewidth}{!}{
%     \begin{tabular}{c|cc|cc}
%     \toprule
%         \multirow{2}{*}{Function} & \multicolumn{2}{|c}{\trial} & \multicolumn{2}{|c}{\NUMOSIM} \\
%         \cline{2-5}
%           & AUROC & AUPR & AUROC & AUPR \\
%          \midrule
%         $\mathcal{L^{\prime}}$ & 0.814  & 0.023  & 0.694 & 0.022 \\
%          \cline{1-5}
%          &   &   &  &   \\
%          \cline{1-5}
%          $\max(\mathcal{L^{\prime}}, \text{kNN})$ & 0.835  & 0.029  &   &   \\
%     \bottomrule
%     \end{tabular}
%     }
% \label{tab:ablation_AD_score}
% \end{table}
% at the event-level (left) and the agent-level (right) anomaly detection
\begin{table}[!th]
    \caption{Comparison of different anomaly scores. $\Delta$, $\alpha$, and $\beta$ denote prediction error, AU, and EU, respectively.  Results demonstrate the effectiveness of incorporating uncertainty estimates and OODness (by kNN) into anomaly scoring.
    % (for numerical features $\Delta_f^{\text{num}}= |\hat{y}_f - y_f|$ and for categorical features $\Delta_f^{\text{cls}}= 1 - p_{f,c}$ where $c$ is the true class). 
    }
    \vspace{-0.1in}
    \centering
    \renewcommand\arraystretch{1.1}
    \setlength\tabcolsep{1 pt}
    \resizebox{1.0 \linewidth}{!}{
    \begin{tabular}{c|cc|cc||cc|cc|cc}
    \toprule
        \multirow{2}{*}{Method} & \multicolumn{4}{c||}{Event-level} & \multicolumn{6}{c}{Agent-level }  \\
        \cline{2-11}
         & \multicolumn{2}{c|}{\trial}& \multicolumn{2}{c||}{\NUMOSIM} & \multicolumn{2}{c|}{\trial} & \multicolumn{2}{c|}{\trialthree} & \multicolumn{2}{c}{\NUMOSIM}  \\
        \cline{2-11}
         & AUROC & AUPR & AUROC & AUPR & AUROC & AUPR & AUROC & AUPR & AUROC & AUPR \\
         \midrule
        $\Delta$   & 0.811  & 0.015 &  \underline{0.711} & \textbf{0.029}  & 0.733  & 0.048  & 0.707 & 0.060 &  0.713 & \underline{0.086} \\
        $\Delta+\alpha+\beta$   &  0.804 & 0.013  & 0.710  & \textbf{0.029}  & 0.689  & 0.034  &  0.738  & 0.106 & 0.701 & 0.075 \\
        $\mathcal{L}^{\prime}$ & \underline{0.814} & \underline{0.023} & 0.694  & \underline{0.022}  & \underline{0.782} &  \textbf{0.094} & \underline{0.824} & \underline{0.194} &  \textbf{0.735} & \textbf{0.090} \\
        $\max(\mathcal{L}^{\prime}, \text{kNN})$ &  \textbf{0.835} & \textbf{0.027} & \textbf{0.740}  & \underline{0.022}  & \textbf{0.790} & \underline{0.091}   & \textbf{0.840} & \textbf{0.202} & \underline{0.723}  & 0.084 \\
    \bottomrule
  
    \end{tabular}
    }
    \label{tab:anomaly_score_ablation}
\end{table}




==> tables/tab_AD_score_func_additional.tex <==

\begin{wraptable}{r}{0.55\linewidth} % 'r' for right, 'l' for left, width of the figure
    \vspace{-0.15in}
    \caption{Results of additional different anomaly scoring functions}
    \vspace{-0.1in}
    \centering
    \renewcommand\arraystretch{1.1}
    \setlength\tabcolsep{2 pt}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{c|cc|cc|cc}
    \toprule
        \multirow{2}{*}{Function} & \multicolumn{2}{|c|}{\trial (small)} & \multicolumn{2}{|c|}{\NUMOSIM(small)} & \multicolumn{2}{|c}{\NUMOSIM(20K)}  \\
        \cline{2-7}
          & AUROC & AUPR & AUROC & AUPR & AUROC & AUPR \\
         \midrule
         $\Delta_f$  & 0.666 & 0.200 & 0.553 & 0.062 & 0.556 & 0.003\\
         \cline{1-7}
         $\text{pth}(\Delta_f)$  & \underline{0.789} & \underline{0.295} & \textbf{0.694} & \underline{0.143} & \underline{0.699} & \underline{0.031} \\
         \cline{1-7}
         $\text{pth}\left(\frac{\Delta_f}{1+\alpha_f+\beta_f}\right)$ & \textbf{0.795} & \underline{0.329} & \textbf{0.694} & \textbf{0.147} & \textbf{0.700} & \textbf{0.034} \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:ablation_AD_score}
    \vspace{-0.1in}
\end{wraptable}

==> tables/tab_AD_score_func_agent.tex <==
\begin{table}% 'r' for right, 'l' for left, width of the figure

    \caption{Comparison of different anomaly scoring functions for agent-level detection.}
    \vspace{-0.1in}
    \centering
    \renewcommand\arraystretch{1.1}
    \setlength\tabcolsep{2 pt}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{c|cc|cc|cc}
    \toprule
        \multirow{2}{*}{Function} & \multicolumn{2}{|c|}{\trial} & \multicolumn{2}{|c|}{\trialthree} & \multicolumn{2}{|c}{\NUMOSIM}  \\
        \cline{2-7}
          & AUROC & AUPR & AUROC & AUPR & AUROC & AUPR \\
         \midrule
        $\mathcal{L^{\prime}}$ & 0.782  & 0.023  &  &  &  &   \\
         \cline{1-7}
          &   &   &  &  &  &   \\
         \cline{1-7}
         $\max(\mathcal{L^{\prime}}, \text{kNN})$ & &  &  &  &  &   \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:ablation_AD_score_agent}
    \vspace{-0.1in}
\end{table}


==> tables/tab_AD_trip_ablation.tex <==

\begin{table}[htbp]% 'r' for right, 'l' for left, width of the figure
    \caption{Comparison of anomaly detection performance w/ or w/o trip features for \trial dataset.}
    \vspace{-0.1in}
    \centering
    \renewcommand\arraystretch{1.1}
    \setlength\tabcolsep{2 pt}
    \resizebox{0.5\linewidth}{!}{
    \begin{tabular}{c|cc|cc}
    \toprule
        \multirow{2}{*}{Function} & \multicolumn{2}{|c}{Event-level} & \multicolumn{2}{|c}{Agent-level} \\
        \cline{2-5}
          & AUROC & AUPR & AUROC & AUPR \\
         \midrule
        w/o trip &  & &  & \\
         \cline{1-5}
         w/ trip & & &  & \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:ablation_trip}
\end{table}


==> tables/tab_ablation.tex <==



\begin{table*}[htbp]
    \caption{Ablation Results on Trial2 dataset.}
    \centering
    \renewcommand\arraystretch{1.1}
    \setlength\tabcolsep{1.5 pt}
    \resizebox{0.7 \linewidth}{!}{
    \begin{tabular}{c|ccccc|cc}
    \toprule
        \multirow{2}{*}{Method} & \multicolumn{5}{|c|}{Masked Prediction} & \multicolumn{2}{|c}{Anomaly Dection}  \\
        \cline{2-8}
         & x@MAE & y@MAE & ST@MAE & SD@MAE & POI@ACC & AUROC & AUPR \\  \midrule
        Dual-Tr-EU & 2.73 & 2.60 & 29.14 & 75.86 & 73.29 & 0.786 & 0.296 \\
        Dual-Tr-AU & 2.46 & 2.36 & \textbf{11.81} & 38.68 & 69.71 & 0.765 & 0.213\\
        Tr-AU-EU  & \textbf{2.33} & \textbf{2.24} & 13.92 & \textbf{34.95} & 73.70 & 0.784 & 0.295 \\ % Tr  AU EU
        Dual-Tr-AU-EU & 2.50 & 2.49 & 12.20 & 37.30 & 70.78 & \textbf{0.795} & \textbf{0.329} \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:ablation}
\end{table*}


% \begin{threeparttable}
% % \resizebox{0.75\linewidth}{!}{


% \begin{tabular}{c|ccc|ccc}
% \toprule
% Downstream Task & \multicolumn{3}{c|}{Travel Time Estimation} & \multicolumn{3}{c}{Destination Prediction} \\
% \midrule
% Methods & RMSE (seconds) & MAE (seconds) & MAPE (\%) & ACC@1 (\%) & ACC@5 (\%) & Recall (\%) \\
% \midrule
% w/o PT & 120.737 $\pm$ 0.634 & 54.951 $\pm$ 2.632 & 12.087 $\pm$ 0.980 & 57.455 $\pm$ 0.723 & 85.331 $\pm$ 0.161 & 28.390 $\pm$ 1.512 \\
% w/o POI & 116.132 $\pm$ 2.131 & 52.941 $\pm$ 4.453 & 12.080 $\pm$ 0.924 & 58.711 $\pm$ 0.215 & 86.128 $\pm$ 0.118 & 29.372 $\pm$ 0.666 \\
% w/o Conv & 117.038 $\pm$ 2.237 & 53.402 $\pm$ 3.175 & \underline{11.836 $\pm$ 1.175} & \underline{59.078 $\pm$ 1.054} & 86.200 $\pm$ 0.673 & 29.521 $\pm$ 1.477 \\
% w/o PSP & 115.454 $\pm$ 5.551 & 53.003 $\pm$ 2.363 & 12.265 $\pm$ 0.856 & 58.797 $\pm$ 0.698 & 86.166 $\pm$ 0.460 & 29.503 $\pm$ 0.779 \\
% w/o $\mathcal{M}$ & \underline{115.233 $\pm$ 0.509} & \underline{52.790 $\pm$ 3.297} & 11.891 $\pm$ 0.794 & 58.930 $\pm$ 0.220 & \underline{86.668 $\pm$ 0.324} & \underline{29.626 $\pm$ 0.287} \\
% PLM4Traj (full) & \textbf{115.079 $\pm$ 1.608} & \textbf{51.973 $\pm$ 1.922} & \textbf{11.635 $\pm$ 0.587} & \textbf{59.594 $\pm$ 0.867} & \textbf{86.740 $\pm$ 0.294} & \textbf{30.184 $\pm$ 0.875} \\
% \bottomrule
% \end{tabular}
% % }
% \begin{tablenotes}\footnotesize
%     \item[]{\textbf{Bold} denotes the best result, and \underline{underline} denotes the second-best result.}
% \end{tablenotes}
% \end{threeparttable}

==> tables/tab_ad_test_dataset.tex <==
\begin{table}[t]%htbp
	\centering
	\caption{Dataset statistics for anomaly detection. The ratio of anomalies depicts the base rate. Note that for \trialthree, the event-level ground truth labels are not provided so there is no event-level evaluation.}
 \vspace{-0.1in}
	\setlength\tabcolsep{2pt}  % Increased padding for better readability
	\resizebox{\linewidth}{!}{  % Ensure it fits within the page width
		\begin{tabular}{lccc}
			\toprule
			& \trial  & \trialthree & \NUMOSIM \\
			\midrule
			\#Agents & 20000 & 20000 & 20,000 \\
			\#Anomalous Agents & 162 & 370 & 381 \\
			Ratio of Anomalous Agents & 0.008 & 0.019 & 0.019 \\
   \midrule
			\#Events & 1,549,104 & 1,794,537 & 1,706,468 \\
			\#Anomalous Events & 892 & - & 3,468 \\
			Ratio of Anomalous Events & 0.0006 & - & 0.002 \\ 

                \midrule

                Time Span & 2 months & 2 months & 2 months \\ 
                City & Los Angeles  & Jordan & Los Angeles \\
                Public/Private & Private  & Private & Public\\ 
   
			\bottomrule
		\end{tabular}
	}
	\label{tab:stat_ad_test_data}
\end{table}


==> tables/tab_agent_level_AD.tex <==
\begin{table*}[htbp]
    \caption{Results of Agent Level Anomaly Detection.}
    \centering
    \renewcommand\arraystretch{1.1}
    \setlength\tabcolsep{2 pt}
    \resizebox{0.6\linewidth}{!}{
    \begin{tabular}{c|cc|cc|cc}
    \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{|c|}{Trial2} & \multicolumn{2}{|c|}{NUMOSIM(small)} & \multicolumn{2}{|c}{NUMOSIM(20k)}  \\
        \cline{2-7}
         & AUROC & AUPR & AUROC & AUPR & AUROC & AUPR \\
         \midrule
         DeepSimple &0.657 & \underline{0.787} & \textbf{0.697} & \textbf{0.638} & 0.703& 0.053\\
         RioBus  & 0.488& 0.632 & 0.510& 0.453& 0.508& 0.019\\
         STOD  & 0.506& 0.655&0.511 &0.468 & 0.519& 0.020\\
         LSTM(v2-max)  &0.631 & 0.706& 0.599& 0.526& 0.658& 0.062\\
         Tr(v2-max)  & \underline{0.679} & 0.785& 0.625 & 0.525 & \underline{0.717} & \underline{0.095}\\
         
         \midrule
         % Dual-Tr-AU-EU(v2) & & & & & & \\
         %Tr-AU-EU(v10-max) &0.757 & 0.829& 0.619 & 0.546 & 0.715 & 0.112\\
         Dual-Tr-AU-EU(v10-max) & \textbf{0.746}& \textbf{0.841}& \underline{0.655}  & \underline{0.572} & \textbf{0.727}& \textbf{0.114}\\
        
    \bottomrule
    \end{tabular}
    }
    \label{tab:agent_anomaly_dection}
\end{table*}

==> tables/tab_anomaly_dection.tex <==



\begin{table*}[htbp]
    \caption{Results of Anomaly Detection.}
    \centering
    \renewcommand\arraystretch{1.1}
    \setlength\tabcolsep{2 pt}
    \resizebox{0.6\linewidth}{!}{
    \begin{tabular}{c|cc|cc|cc}
    \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{|c|}{Trial2} & \multicolumn{2}{|c|}{NUMOSIM(small)} & \multicolumn{2}{|c}{NUMOSIM(20k)}  \\
        \cline{2-7}
         & AUROC & AUPR & AUROC & AUPR & AUROC & AUPR \\
         \midrule
         DeepSimple & 0.593 & 0.221 & 0.630& \underline{0.144} & 0.634& 0.008 \\
         RoiBus & 0.503 & 0.044 & 0.530 & 0.047 & 0.532 & 0.002\\
         STOD & 0.577 & 0.073 & 0.571 & 0.071 & 0.584 & 0.003\\
         LSTM & \underline{0.755} & 0.182 & \underline{0.637} & 0.122 & \underline{0.642} & 0.020\\
         Tr & 0.723 & \underline{0.232} & 0.635 & 0.132 & 0.636 & \underline{0.033} \\
         
         \midrule
         % Dual-Tr-AU-EU(v2) & & & & & & \\
         %Tr-AU-EU & \underline{0.784} & \underline{0.295} & \underline{0.693} & \underline{0.156} & \textbf{0.696} & \underline{0.040}\\
         Dual-Tr-AU-EU & \textbf{0.795} & \textbf{0.329} & \textbf{0.694} & \textbf{0.146} & \textbf{0.670} & \textbf{0.034}\\
        
    \bottomrule
    \end{tabular}
    }
    \label{tab:event_anomaly_dection}
\end{table*}



==> tables/tab_injection_AD_2.tex <==
\begin{table}% 'r' for right, 'l' for left, width of the figure
    \caption{Anomaly detection results at event level using loss or KNN for datasets of different types of injected anomalies.}
    \vspace{-0.1in}
    \centering
    \renewcommand\arraystretch{1.1}
    \setlength\tabcolsep{2 pt}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{c|cc|cc|cc}
    \toprule
        \multirow{2}{*}{Injection Type} & \multicolumn{2}{|c|}{Loss} & \multicolumn{2}{|c|}{KNN} & \multicolumn{2}{|c}{Loss \& KNN}  \\
        \cline{2-7}
          & AUROC & AUPR & AUROC & AUPR & AUROC & AUPR \\
         \midrule
         Spatial  &  &  &   &   &    &   \\
         \cline{1-7}
         Temporal &  &  &   &   &    &   \\
         \cline{1-7}
         Spatial \& Temporal&  &  &   &   &    &   \\
         \cline{1-7}
         Swap &  &  &   &   &    &   \\
         \cline{1-7}
         Permutation &  &  &   &   &    &   \\
         \cline{1-7}
         High-density &  &  &   &   &    &   \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:ablation_injection_2}
    \vspace{-0.1in}
\end{table}


==> tables/tab_masked_pred_AD_trip.tex <==
\begin{table}[htbp]
\centering
\small
\caption{Masked prediction results (left) and anomaly detection results (right) for \method~w/ or w/o trip features on \trial. We \textbf{bold} the best performance and \underline{underline} the second best. Abbr: ST; start time (min), SD; stay duration (min), x, y; lat/lon (km). W/ trip improves the prediction performance for spatial features. }
\vspace{-0.1in}
\renewcommand\arraystretch{1.1}
\setlength\tabcolsep{2 pt}
\resizebox{1.0 \linewidth}{!}{

\begin{tabular}{c|cccc|cccc|c||cc|cc}
\toprule %\hline
\multirow{3}{*}{Method}
% & \multicolumn{12}{|c|}{Trial2}& \multicolumn{12}{|c}{NUMOSIM} \\
& \multicolumn{9}{|c||}{Masked Prediction}  & \multicolumn{4}{c}{Anomaly Detection} \\
\cline{2-14}
& \multicolumn{4}{|c}{MAE}& \multicolumn{4}{|c}{MAPE (\%)}& \multicolumn{1}{|c||}{ACC(\%)} & \multicolumn{2}{c}{Event-level}& \multicolumn{2}{|c}{Agent-level} \\
\cline{2-14}
 & x & y & ST & SD &  x & y & ST & SD & POI & AUROC & AUPR & AUROC  & AUPR \\
\midrule %\hline

w/o trip  & 2.4 & 2.3 & 11.4 & 35.8 & 109.4 & 102.5 & 15.9 & 20.9 & 73.0 & &  &  &  \\ \hline
w/ trip & 0.64 & 0.63 & 13.2 & 45.9 & 34.0 & 33.3 & 15.4 & 31.2 & 73.6 & & & &\\ \hline

\bottomrule

\end{tabular}
}

\label{tab:masked_pred_AD_trip}
\end{table}

==> tables/tab_masked_prediction_in_main.tex <==
\begin{table}[htbp]
\centering
\small
\caption{Masked prediction results. We \textbf{bold} the best performance and \underline{underline} the second best. Abbr: ST; start time (min), SD; stay duration (min), x, y; lat/lon (km). \method significantly outperforms the baselines with the uncertainty modeling ability, while allowing conformal prediction.}
\vspace{-0.1in}
\renewcommand\arraystretch{1.1}
\setlength\tabcolsep{2 pt}
\resizebox{1.0 \linewidth}{!}{
% \begin{tabular}{c|cccccc|cccccc|cccccc|cccccc}
\begin{tabular}{c|cccc|cccc|c}
\toprule %\hline
\multirow{3}{*}{Method}
% & \multicolumn{12}{|c|}{Trial2}& \multicolumn{12}{|c}{NUMOSIM} \\
& \multicolumn{9}{|c}{\trial}  \\
\cline{2-10}
& \multicolumn{4}{|c|}{MAE}& \multicolumn{4}{|c|}{MAPE (\%)}& \multicolumn{1}{|c|}{ACC(\%)} \\
\cline{2-10}
 & x & y & ST & SD &  x & y & ST & SD & POI   \\
\midrule %\hline

MLP \citep{MLP}  & 9.73 & 10.16 & 208.07 & 420.92 & 188.13 & 500.59 & 43.28 & 569.01 & 45.61    \\ \hline
LSTM \citep{LSTM} & 4.73 & 4.63 & 19.85 & 322.62 & 204.73 & 195.76 & 18.25 & 420.76 & 63.32   \\ \hline

Transformer \citep{Transformer} & 2.67 & 2.65 & 26.85 & 77.12 & 132.33 & 115.35 & 17.95 & 66.82 & 73.49   \\ \hline

%SensitiveHUE\cite{Feng2024HUE} &  & &  &  &  &  &   &  & -   \\ \hline

Dual-Tr & 2.71 & 2.63 &  20.62 & 76.53 & 131.72 & 117.29  & 16.41 & 51.95 & \underline{73.74}  \\ 

% \citep{MLP}, LSTM \citep{LSTM}, the original Transformer \citep{Transformer}
%Tr-AU-EU & 2.33 & 2.24 & 13.92 & 34.95 & 111.69 & 102.05 & 15.49 & 20.93 & 73.70 & 3.32 & 3.15 & 27.58 & 36.40 & 121.86 & 67.19 & 246.13 & 26.18 & 76.44  \\ \hline

\midrule \hline

% Dual-Tr-AU-EU & \textbf{2.50} & \textbf{2.49} & \textbf{12.20} & \textbf{37.30} & \textbf{111.75} & \textbf{102.35} & \textbf{13.88} & \textbf{18.04} & 70.78 & \underline{3.70} & 3.62 & 27.04 & \textbf{46.17} & \textbf{122.64} & 83.98 & 236.57 & \textbf{29.54} & 74.30\\ \hline


\method & \underline{2.44} & \underline{2.29} & \underline{11.42} & \underline{35.77} & \underline{109.44} & \underline{102.47} & \underline{15.86} & \underline{20.93} & 72.97   \\


% Dual-Tr-AU-EU(2\%) & 2.26 & 2.11 & 9.21 & 27.23 & 104.45 & 97.48 & 1.24 & 20.73 & 74.10 & 3.47 & 3.41 & 13.67 & 39.02 & 112.05 & 76.66 & 53.24 & 28.68 & 75.44 \\

% Dual-Tr-AU-EU(3\%) & 2.17 & 2.03 & 9.00 & 25.22 & 101.83 & 94.63 & 1.22 & 20.68 & 74.60 & 3.41 & 3.34 & 9.11 & 36.88 & 111.12 & 76.17 & 1.53 & 28.73 & 75.94 \\

\method(5\%) & \textbf{2.05} & \textbf{1.91} & \textbf{8.65} & \textbf{21.98} & \textbf{99.39} & \textbf{89.45} & \textbf{1.18} & \textbf{20.66} & \textbf{75.58}   \\



\bottomrule


% baseline stat: trial 2 poi acc = 0.4561; NUMOSIM poi ACC = 0.560
% for trial2: during 9 to 5, random.sample(office,store), otherwise home; for NUMOSIM: during 9 to 5, randomly sample from previous top 2 most frequent POI, otherwise home

\end{tabular}
}

\label{tab:masked_prediction}
\end{table}

==> tables/tab_uc_train_data_relation_main.tex <==
\begin{table}[htbp]
\centering
\vspace{-1em}
\caption{AU and EU for x and POI under different training data size settings. As training data increase, AU stays steady while EU decreases noticeably.}
\vspace{-0.5em}
\resizebox{0.9 \linewidth}{!}{%
\begin{tabular}{c|c|c|c|c|c}
\toprule
Train & Test & \multicolumn{2}{c|}{x} & \multicolumn{2}{c}{POI} \\
\midrule
      &      & AU $\times 10^{-3}$ & EU $\times 10^{-5}$ & AU $\times 10^{-2}$ & EU  $\times 10^{0}$ \\
\midrule
1-week & 2-week & 1.57 & 1.31 & 3.47 & 1.18 \\
2-week & 2-week & 1.92 & 1.19 & 3.13 & 1.14 \\
3-week & 2-week & 1.34 & 0.71 & 4.47 & 1.09 \\
\bottomrule
\end{tabular}%
}
\label{tab:uc_train_data_relation}
\end{table}

